APEX: A Network-Native Time-Series Foundation Model for Forecasting and Anomaly Detection for Wireless Edge Operations

Generic time-series foundation models transfer poorly to wireless network telemetry whose signals are bursty, zero-inflated, and coupled across protocol layers. We present APEX, a network-native, decoder-only transformer for forecasting enterprise AP telemetry, and evaluate it on DHCP degradation as a representative network task. APEX is pre-trained on 10-channel multivariate telemetry from ~4,500 production wireless networks (~100K AP time series, 34 metrics per AP), and is available as APEX-Large (269M, cloud) and APEX-Edge (10.5M, edge). On a 192-step (4-day) DHCP degradation benchmark, APEX-Large reduces MAE by 18% over the strongest foundation-model baseline (Toto) and 38% over SARIMA, with anomaly-detection F1 = 0.93, while APEX-Edge enables sub-second, privacy-preserving inference on AP-class edge hardware. These results suggest network-native pre-training is a practical foundation for proactive wireless operations.

==> sections/background.tex <==
\section{Background and Motivation}
\label{sec:background}

\textbf{Why network telemetry is different.}
Access points simultaneously observe Layer~2/3 protocol transactions (DHCP discover/offer/request/ACK cycles), RF physical measurements (SNR, channel utilization, noise floor), transport-layer performance (throughput, packet loss), and topology state (client count, server count, VLAN count).
These signals are \emph{co-collected}, sampled from the same device at the same timestamps, and \emph{co-located}, measuring the same physical and logical network segment.
This co-collection preserves temporal alignment and causal relationships between protocol layers that are lost when telemetry is aggregated across heterogeneous collection pipelines.

Four properties distinguish this data from public time-series benchmarks:

\textbf{(1) Extreme sparsity with bursty events.}
DHCP failure counts are zero during normal operation and spike during incidents.
The distribution is zero-inflated with heavy tails, a regime poorly served by models pretrained on smooth, continuous data.

\textbf{(2) Protocol-specific temporal structure.}
DHCP transactions follow a discover$\to$offer$\to$request$\to$ACK state machine with characteristic timing.
A spike in discover rate followed by a drop in offer rate (with a specific lag) indicates server exhaustion, not random noise.

\textbf{(3) Cross-layer causal chains.}
RF degradation (SNR drop) causes client disassociations, which trigger DHCP re-discoveries, which may overwhelm servers, causing NACK spikes.
This chain spans three feature groups and unfolds over minutes to hours.

\textbf{(4) Topology-dependent dynamics.}
The relationship between client count and DHCP latency is mediated by server count and VLAN configuration, topology descriptors that modulate dynamics in network-specific ways.

\textbf{Why edge deployment demands domain-specific models.}
Privacy-sensitive enterprise environments increasingly require that raw telemetry never leave the AP.
General-purpose foundation models (TimesFM at 200M, Toto at 151M, Chronos-2 at 120M parameters) are too large for AP-class hardware and require cloud inference, introducing latency and a WAN dependency that defeats the purpose of predictive, preemptive action.
A domain-specific model can be made smaller \emph{because} it encodes network priors directly, rather than reserving capacity for weather, finance, and energy dynamics it will never encounter at the edge.


==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}

\textbf{Domain-specific pretraining is necessary, not optional.}
The consistent gap between APEX-Large and general-purpose models is not an architecture effect; both use decoder-only transformers with patching.
It is a \emph{data} effect: network telemetry has statistical properties (zero-inflation, protocol state machines, cross-layer causality) that are absent from public pretraining corpora.
We conjecture this finding generalizes: any vertical domain with sufficiently distinctive data distributions will benefit from domain-specific foundation models over zero-shot transfer from general-purpose ones.

\textbf{Multivariate structure matters.}
The APEX-Large (multi) vs.\ APEX-Large (1D) ablation isolates the value of cross-channel attention at full capacity.
The APEX-Edge (multi) vs.\ APEX-Edge (1D) comparison tests whether this benefit persists under aggressive compression.
The causal chain structure of DHCP metrics provides genuine Granger-causal signal that multivariate models exploit.
This is not guaranteed for arbitrary metric bundles; the choice of which channels to co-model is a domain design decision, not a free lunch.

\textbf{Size--accuracy tradeoff.}
The $2{\times}2$ ablation (large/small $\times$ 1D/multi) characterizes the Pareto frontier between model capacity and forecasting accuracy.
APEX-Edge (10.5M) is 26$\times$ smaller than APEX-Large (269M); quantifying the accuracy gap between them informs deployment decisions about when cloud inference is justified versus when edge-only operation suffices.

\textbf{Privacy-preserving edge inference.}
APEX-Edge demonstrates that domain-specific pretraining enables aggressive compression.
This is the key enabler for privacy-preserving deployment: raw telemetry stays on-device, and only anomaly flags traverse the network.
For regulated industries, this is not a nice-to-have but a deployment prerequisite.

\textbf{Limitations.}
Our evaluation uses consensus pseudo-labels rather than human-annotated ground truth.
Edge latency is measured on a Raspberry Pi~5 proxy, not production AP hardware.
APEX-Large requires cloud inference; APEX-Edge trades some accuracy for deployability.
Full characterization of this tradeoff across both input modes (Table~\ref{tab:forecast}) is in progress.

